Art and Science Interaction Lab -- A highly flexible and modular interaction science research facility

The Art and Science Interaction Lab (ASIL) is a unique, highly flexible and modular interaction science research facility to effectively bring, analyse and test experiences and interactions in mixed virtual/augmented contexts as well as to conduct research on next-gen immersive technologies. It brings together the expertise and creativity of engineers, performers, designers and scientists creating solutions and experiences shaping the lives of people. The lab is equipped with state-of-the-art visual, auditory and user-tracking equipment, fully synchronized and connected to a central backend. This synchronization allows for highly accurate multi-sensor measurements and analysis.

==> 5_discussion.tex <==
%%%%%%%%%%%%%%
% DISCUSSION %
%%%%%%%%%%%%%%

\section{Discussion}

The main motivation behind the development of this framework was to combine ease of use and the need to gain deeper insights during WoZ user tests. The proposed system not only allows the researcher to create tests easily, but data processing is automated as well. The outcome is a useful tool for testing systems that are difficult to build prototypes of in real life. An example of such prototypes mentioned often in this paper are smart systems containing IoT devices. These can be simulated easily in VR to work, but are more difficult to prototype working in real life. These simulations are often positioned in the domain of user testing and training applications. We believe our approach and tool have several advantages over other similar methodologies. Where current usertesting demands physical space, objects and people, VR usertesting is possible in a virtual space with virtual objects and people. This results in a faster workflow, a smaller development cost and more versatility by using online databases.The automatic logging of HCCI events is another benefit. Since interactions are performed in a virtual world, all the data can be tracked in real time and can be synced with the measured physio data. The last benefit of a virtual testing service is viewing and replaying the actions of participants from all possible angles.

In sum, we believe that the proposed system is a great step forward for interactive user testing of smart systems. Furthermore, an early validation of  the framework is described in this paper by performing a pilot test on the use case of a smart kitchen environment.


==> 5_results.tex <==
%%%%%%%%%%%
% RESULTS %
%%%%%%%%%%%

\section{Results}
%description and justification of procedure and/or results
This pilot study was performed to have a first impression on the use of the developed system. It serves as a proof of concept but also shows which aspects of the platform still need work. The brief usability test combined with a semi structured interview delivers deeper insights in the usability perceived by the users. It also indicates if the selected 'wizard' uses alternative workflows when operating the dashboard. 

In the next paragraph you can read a detailed description on the experience of the wizard (designer) and the participant (end user). A detailed evaluation of the usability of this system with a larger sample size will follow in a next publication.

%visual?


%general findings


%detailed findings
\subsection{Subjective experience of the prototyper/designer}

\subsubsection{UTAUT and SUS}
The semi structured interview used questions from the UTAUT and SUS framework combined with in-depth questions on the functionality of the different parts of the dashboard.



%Performance expectancy



During the interview afterwards, the 'wizard' indicated that she found the system easy to use but still needs some technical support to start using it. She thinks that people will find out how to use it quite quickly. The different functionalities of the system were well integrated. After trying it out the second time, she felt confident while using the system.


A more clear onboarding and introduction to the system would be preferred. As chances to conduct a good test increase if the technology works well and the system is easy to operate by yourself without technical support when you know have learned how it works. This is especially true for testing new concepts that don’t exist yet and bigger projects (for example: escape games, public spaces, smart device interactions). These are generally hard to recreate in a Wizard of Oz test.The system is not well suited for highly realistic multi sensory experiences or smaller projects (like cooking or other detailed multi sensory actions). The designer who evaluated the wizard interactions, praised the versatility of VR as it can be used to conduct the same experiment over and over again or to have a slightly different experiment every time. The VR dashboard not only gave an indication whether people will use the tested product correctly but also gives insight whether they like the interactions with the tested product.She also commented that the persons who will support the use of this system are primarily educators and employers in all domains that are related to user testing.



%effort expectancy
Even though the system was perceived as easy to use, some functionality problems remained. Some functionalities were not noticed by the first time use (for example a button for switching the tablet with the voice assistant). The system seemed easy to become competent in except for very technical features (such as displacing the avatar or viewport cameras). Anticipating behaviour of the participant still remains hard. When this goes wrong, there is also a risk that something unnatural can happen during a user test (for example actions toggled on too soon, or frustration from the participant when the wizard reacts too late or not at all). 

In her opinion, the system could be improved if the wizard is able to hear what the participant hears at all times. Another useful adaptation would be a shadow mode where the wizard can prepare interactions before activating them for the participant. At this point in time,  the wizard and participant see the same scene at all times right now. Asynchronous interactions could alleviate the load of the wizard during the user test. The cost of the VR setup and limited knowledge of programming were argued to limit the accessibility of this system for many test designers.

%behavioural intention
Regarding future use, The designer commented that she would like to test the system in different phases and for different user profiles (ranging from early adopters to late majority of product users). This could be done at a few given times in the development process (concept definition, early prototypes and interface design).

It was not clear yet to the wizard how the data from the experiment could be used. It could be useful for post analysis (of large samples). First, you can see in the data when something in the experiment went wrong. Second, you can test if one scenario works better than another. You could even see if data collection went wrong in an experiment by doing certain queries since a lot of different data is captured. The wizard found it interesting to look into the data of one interaction of one participant, but also of multiple interactions (sequence) of multiple participants. or even combinations between the two (ratio between interactions compared in different participants)

%SUS

\subsubsection{Specific questions on different functionalities of the system} 
% specific Questions on different functionalities of the system
The wizard liked the integration of the scene control and general control buttons. Still user friendliness can be increased. She suggested using icons instead of text so you can toggle buttons but do not need to read them each time). 
The designer commented that she was eager to learn how to create her own buttons to trigger actions in future experiments. If possible, coding should be avoided and drag-and-drop or a library of prefabricated solutions should help designers implement control buttons in future projects.

According to the designer, the Wizardview was an interesting feature. However it remains impossible to read body language as in real life, since the tracking is not accurate enough. The secondary camera allows the wizard to get a good overview and see objects that are out of the participant's view.

The interaction data can be useful for probing and realtime interpretations. Behaviour can be triggered to draw live conclusions. It can be studied if the VR environment and setup gave participants stress even before experiments started. Another similar example is that the wizard can see if text was hard too read for a participant if he looks at the text for too long. (mistakes or exceptionally long gaze times can be found in the data).

% perception of actions was realistic?

%look and feel
%usability
%problems
%opportunities

\subsection{Subjective experience of the end user}
During the interview afterwards, the participant indicated that the tasks in VR were sufficiently developed to do an assessment of the functionalities when using the interface of a tablet compared to the interface of a voice assistant in the kitchen. The participant commented that it was unclear which actions he could and could not do in the kitchen. Some examples of actions that were not implemented were cutting vegetables and using the oven.

Regarding the quality of experience, the participant commented that he felt immersed in the VR world. The environment was not really realistic, but this was not a problem for evaluation of the tablet and Alexa. Timing how long steps take can be different compared to real life. For example, filling the pot with water goes instantly. When asked about feeling present in VR the participant commented that he felt immersed in VR. The participant mentioned that the adaptation went quickly even though he had some problems with focus, nausea and a small headache. The participant mentioned some issues with the hand held controllers. This indicates that user testing could benefit from more realistic interactions in VR (, because then such confusion would not happen). 

The participant did not feel that there was a 'Wizard' controlling his actions afterwards it became clear to him that most interaction he did (filling a pot with water, baking bacon on the stove, controlling the tablet) were done by the 'wizard'. The participant was quite willing to wear all peripherals needed for the test (headset, battery, heart rate sensor).
